InfoNCE is variational inference in a recognition parameterised model

Here, we show that the InfoNCE objective is equivalent to the ELBO in a new class of probabilistic generative model, the recognition parameterised model (RPM). When we learn the optimal prior, the RPM ELBO becomes equal to the mutual information (MI; up to a constant), establishing a connection to pre-existing self-supervised learning methods such as InfoNCE. However, practical InfoNCE methods do not use the MI as an objective; the MI is invariant to arbitrary invertible transformations, so using an MI objective can lead to highly entangled representations (Tschannen et al., 2019). Instead, the actual InfoNCE objective is a simplified lower bound on the MI which is loose even in the infinite sample limit. Thus, an objective that works (i.e. the actual InfoNCE objective) appears to be motivated as a loose bound on an objective that does not work (i.e. the true MI which gives arbitrarily entangled representations). We give an alternative motivation for the actual InfoNCE objective. In particular, we show that in the infinite sample limit, and for a particular choice of prior, the actual InfoNCE objective is equal to the ELBO (up to a constant); and the ELBO is equal to the marginal likelihood with a deterministic recognition model. Thus, we argue that our VAE perspective gives a better motivation for InfoNCE than MI, as the actual InfoNCE objective is only loosely bounded by the MI, but is equal to the ELBO/marginal likelihood (up to a constant).

==> resubmission_text.tex <==
This is a resubmission of submission #449 "InfoNCE is a variational autoencoder".

This resubmission is becoming increasingly urgent as a subfield is being built upon the contributions of our original paper.  We have included an extensive discussion of this work building on our original submission in the Related work section.  This work includes:

* William I Walker, Hugo Soulat, Changmin Yu, and Maneesh Sahani. Unsupervised representational learning with recognition-parametrised probabilistic models. AISTATS, (2023a)
* William I. Walker, Arthur Gretton, and Maneesh Sahani. Prediction under latent subgroup shifts with high-dimensional observations. arXiv (2023b)
* Yu Wang, Hengrui Zhang, Zhiwei Liu, Liangwei Yang, and Philip S Yu. Contrastvae: Contrastive variational autoencoder for sequential recommendation. In Proceedings of
the 31st ACM International Conference on Information & Knowledge Management 2022.
* Arman Hasanzadeh, Mohammadreza Armandpour, Ehsan Hajiramezanali, Mingyuan Zhou, Nick Duffield, and Krishna Narayanan. Bayesian graph contrastive learning. 2021.
* Adam Jelley, Amos Storkey, Antreas Antoniou, and Sam Devlin. Contrastive meta-learning for partially observable few-shot learning. 2023.

In the previous submission, after extensive discussion the reviewers agreed unanimously that the paper should be published:

ZXW3:

* The main idea of the paper is written clearly, with all derivations and assumptions explicitly stated.
* The theoretical contribution that links VAE with InfoNCE is correct, novel (to my knowledge), interesting and significant. In particular, the analyses in 3.6 is elegant and give me a good thrill.
* The experiment clearly makes the point that prior choice is crucial.

cHbB:

* The new connection between InfoNCE and SSVAEs is novel and interesting.

McsS:

* Update: the authors have made several changes to the earlier writing which I think clarifies quite a bit, as well as renaming the model they consider. While I still feel this work could benefit from additional rewriting, at this point I would consider it above the bar for publication at TMLR.

5HXJ:

* (I don't challenge the math derivations), but I think the interpretation of the math (the writing) can be made clearer

Surprisingly, the AE rejected the paper, based on novel comments that were not brought up during the original and would have been easy to rectify in a revision.  These objections are largely obviated by the follow-up work discussed above (especially Walker 2023a).

Nonetheless, we discuss each of the points in turn here,

> The paper makes several problematic claims. The key claim that the paper shows that contrastive SSL methods "implicitly learn a full probabilistic model of the inputs" parameterized as a VAE, does not hold up. The likelihood of this "probabilistic model" is defined as P(x|z) = Q(z|x)P_true(x)/Q(z), which means it depends not only on the intractable aggregate variational posterior Q(z) but also on the unknown true data distribution P_true(x). This means that we can neither evaluate nor sample from the likelihood/model (even using MCMC), so this construction does not define a proper model, not even an implicit one. Calling such a "model" a "VAE" is done in the title of the paper is even less accurate.

We have considerably modified the paper, to point out that:
* In an empicical marginal RPM, you can sample.
* Sampling isn't the point (as in other probabilistic generative models models such as Latent Dirichlet Allocation, probabilistic PCA and others).

> The claim that "when we learn the optimal prior, the VAE objective (the ELBO) becomes equal to the MI" is not quite right either because it fails to mention another term in the objective, which does not depend on the encoder parameters.

we have added "up to a constant" where applicable.

> The claim that "for a deterministic encoder the ELBO is equal to the log Bayesian model evidence" is true, but it is not novel and is not shown rigorously in the paper. The problematic fact that such an encoder results in an infinite KL(q(z|x)||p(z)) term in the ELBO is not acknowledged or addressed. To derive the result rigorously, one can take the limit of the encoder variance going to zero as was done in SurVAE Flows paper [1]. Note that such a model with a deterministic encoder is not a VAE.

We have added a new Appendix on the measure theory underlying these results.


> The implication in the experimental section that the choice of Gaussian-PDF-like function f which worked well was somehow less natural from the InfoNCE SSL perspective (compared to the advocated generative one) is highly debatable. For example, the difference between using Eq. 39 and Eq. 40 becomes considerably smaller if z and z' in Eq. 39 are restricted to be unit norm, as is often done in self-supervised representation learning. Including this version of f in the very minimal experimental section could provide more evidence for the claim being made.

While restricting to a unit-norm is common, it does not seem particularly well-motivated in a MI setting, as projecting down to a hypersphere will necessarily reduce the MI (as we're pushing z through a many-to-one transformation from a D dimensional Euclidean manifold to a D-1 dimensional manifold).



